Antenna subtraction at NNLO with hadronic initial states: double real radiation for initial-initial configurations with two quark flavours

The antenna subtraction formalism allows to calculate QCD corrections to jet observables. Within this formalism, the subtraction terms are constructed using antenna functions describing all unresolved radiation between a pair of hard radiatior partons. In this paper, we focus on the subtraction terms for double real radiation contributions to jet observables in hadron-hadron collisions evaluated at NNLO. An essential ingredient to these subtraction terms are the four-parton antenna functions with both radiators in the initial state. We outline the construction of the double real subtraction terms, classify all relevant antenna functions and describe their integration over the relevant antenna phase space. For the initial-initial antenna functions with two quark flavours, we derive the phase space master integrals and obtain the integrated antennae.

==> M1.tex <==
\begin{align}
% MR 10.1.2011: k_a -> k_j, k_b -> k_k
\I{1} \times k_k \cdot p_1 \;\;&=I_1 = 
(s_{12})^{1 - 2 \ep}
\frac{N_{\Gamma}\, (1-x_1)^{-2 \ep}\,
(1-x_2)^{-2 \ep}}{8\, (x_1+x_2)^2} \,\times
\nonumber \\
&
\Bigl[
-(x_1-1) (x_2-1)^2 (x_2 x_1+2 x_1+x_2)
\nonumber \\
&
+\ep\;\Bigl\{(x_1-1) (x_2 x_1+2 x_1+x_2) \text{H}(0,x_1) (x_2-1)^2
-\frac{1}{2} (x_1-1) \,\times
\nonumber \\
&
\left(5 x_1 x_2^2+3 x_2^2+3 x_1 x_2-7 x_2-12 x_1\right) (x_2-1)
\nonumber \\
&
-2 \left(x_1^2 x_2^3-x_2^3-2 x_1 x_2^2-3 x_1^2 x_2-x_2-2
x_1\right) \text{G}(-x_2,x_1)
\nonumber \\
&
+(x_1+1) (x_2+1)^2 (x_2 x_1-2 x_1-x_2) (\text{H}(-1,x_1)+\text{H}(-1,x_2)
\nonumber \\
&
-\text{H}(0,x_2))+4 (x_1+x_2)^2 \log (2)\Bigr\}
\nonumber \\
&
+\ep^2\;\Bigl\{+(x_1-1) (x_2 x_1+2 x_1+x_2)
(\text{H}(0,-1,x_2)-\text{H}(0,0,x_1)-\text{H}(0,0,x_2)) \,\times
\nonumber \\
& 
(x_2-1)^2-\frac{9}{4} (x_1-1) \left(3 x_1 x_2^2+x_2^2+x_1 x_2-5 x_2-8
x_1\right) (x_2-1)
\nonumber \\
& 
+\frac{1}{2} (x_1-1) \left(5 x_1 x_2^2+3 x_2^2+3 x_1 x_2-7 x_2-12
x_1\right) \text{H}(0,x_1) (x_2-1)
\nonumber \\
& 
+\left(-5 x_1^2 x_2^3+3 x_2^3+8 x_1 x_2^2+15 x_1^2 x_2+7 x_2+12
x_1\right) \text{G}(-x_2,x_1)
\nonumber \\
&
+\left(x_1^2 x_2^3-x_2^3-2 x_1 x_2^2-3 x_1^2 x_2-x_2-2 x_1\right)
(2 \text{G}(0,-x_2,x_1)
\nonumber \\
& 
+2 \text{G}(-x_2,-1,x_1)
+2 \text{G}(-x_2,0,x_1)-4 \text{G}(-x_2,-x_2,x_1)
\nonumber \\
& 
+\text{G}(-x_2,x_1) (2 \text{H}(-1,x_2)-2 \text{H}(0,x_2)))+(x_1+1) (x_2+1) 
\,\times
\nonumber \\
& 
\left(5 x_1 x_2^2-3 x_2^2-3 x_1 x_2-7 x_2-12
x_1\right) \left(\frac{1}{2} \text{H}(-1,x_1)+\frac{1}{2} \text{H}(-1,x_2)
\right.\nonumber \\
& \left.
-\frac{1}{2} \text{H}(0,x_2)\right)+\left(-x_1^2 x_2^3+x_2^3+2 x_1 x_2^2+6
x_2^2+3 x_1^2 x_2+12 x_1 x_2
\right.\nonumber \\
& \left.
+x_2+6 x_1^2+2 x_1\right)
(\text{G}(1,-x_2,x_1)+\text{H}(-1,x_2) \text{H}(1,x_1)+\text{H}(1,-1,x_1)
\nonumber \\
& 
+\text{H}(1,-1,x_2))+\left(x_1^2 x_2^3-x_2^3-2 x_1 x_2^2-6 x_2^2-3 x_1^2
x_2-12 x_1 x_2
\right.\nonumber \\
& \left.
-x_2-6 x_1^2-2 x_1\right) (\text{H}(0,x_2) \text{H}(1,x_1)+\log
(2) \text{H}(1,x_1)+\text{H}(1,0,x_2)
\nonumber \\
& 
+\text{H}(1,x_2) \log (2))+(x_1+x_2)^2 \left(-4 \log
(2) \text{H}(0,x_1)-4 \log ^2(2)
\right.\nonumber \\
& \left.
-4 \text{H}(0,x_2) \log (2)\right)+(x_1+1) (x_2+1)^2 (x_2 x_1-2 x_1-x_2) \,\times
\nonumber \\
&
\left(3 \text{G}(-1,-x_2,x_1)+\text{H}(0,x_1) \text{H}(0,x_2)
-2 \text{H}(-1,-1,x_1)
\right.\nonumber \\
& \left.
-2 \text{H}(-1,-1,x_2)-\text{H}(-1,0,x_1)+2 \text{H}(-1,0,x_2)-\text{H}(0,-1,x_1)
\right.\nonumber \\
& \left.
+\text{H}(-1,x_2) (\log (2)-\text{H}(0,x_1))+\text{H}(-1,x_1)
(-2 \text{H}(-1,x_2)
\right.\nonumber \\
& \left.
+2 \text{H}(0,x_2)+\log (2))+\frac{\pi ^2}{3}\right)
\nonumber \\
&
-2 (x_1+x_2) \left(x_1x_2^2-5 x_2-6 x_1\right) \log (2)\Bigr\}
+ \mathcal{O}(\ep^3)\; \Bigr]\,.
\end{align}


==> M10.tex <==
\begin{align}
\I{10} \;\;&=I_{10} =  
(s_{12})^{-1 - 2 \ep}
\frac{(1-2 \,\ep)\, N_{\Gamma}\, (1-x_1)\,^{-2 \,\ep}
(1-x_2)\,^{-2 \,\ep}}{x_1} \, \times
\nonumber \\ 
&\Bigl[ \,\text{G}(-x_2,x_1)\,-\,\text{H}(-1,x_2)\,+\,\text{H}(0,x_2)\,
+\,\ep \;\Bigl\{-\,\text{G}(0,-x_2,x_1)\,
\nonumber \\
&
+2 \,\text{G}(1,-x_2,x_1)\,
%\right. \right. \nonumber \\&
-\,\text{G}(-x_2,-1,x_1)\,-\,\text{G}(-x_2,0,x_1)\,+2 \,\text{G}(-x_2,-x_2,x_1)\,
\nonumber \\
&
-\,\text{H}(0,x_1)\, \,\text{H}(0,x_2)\,
+\,\text{G}(-x_2,x_1)\, (-\,\text{H}(-1,x_2)\,+\,\text{H}(0,x_2)\,+2)\,
\nonumber \\
&
+\,\text{H}(0,x_2)\, (-2 \,\text{H}(1,x_1)\,
-2 \,\text{H}(1,x_2)\,+2)\,
+2 \,\text{H}(-1,-1,x_2)\,
\nonumber \\
&
-2 \,\text{H}(-1,0,x_2)\,-2 \,\text{H}(-1,1,x_2)\,
+2 \,\text{H}(0,1,x_2)\,-3 \,\text{H}(1,-1,x_2)\,
%%%%%\nonumber \\ & \left. \left.
\nonumber \\
&
+3 \,\text{H}(1,0,x_2)\,
+\,\text{H}(-1,x_2)\, (\,\text{H}(0,x_1)\,
+2 \,\text{H}(1,x_1)\,
+2 \,\text{H}(1,x_2)\,
\nonumber \\
&
+\log (2)\,-2)\,
+\,\text{H}(1,x_2)\, \log (2)\,-\frac{\pi ^2}{4}\Bigr\} + \mathcal{O}(\,\ep^2)\,\Bigr]\,. 
\end{align}



==> M14.tex <==
\begin{align} 
\label{M14hard}
\I{14} \;\;&=I_{14} = 
(s_{12})^{-2 - 2 \ep}
\left( -\frac{N_{\Gamma}}{b\,s\, x_1\, x_2\,} \right)
\,\times
\nonumber \\
&
 \Bigl[\,\log \left(\frac{1+\,s}{1-\,s}\right) \left(\log \left(\frac{-b\,s-x_{12\,}+2\,}{b-x_{12\,}+2\,}\right)+\log \left(\frac{b\,s-x_{12\,}+2\,}{b-x_{12\,}+2\,}\right)\right)
\nonumber \\
&
-\log \left(\frac{b\,s-x_{12\,}+2\,}{-b\,s-x_{12\,}+2\,}\right) \log \left(\frac{b+x_{12\,}-2\,}{b-x_{12\,}+2\,}\right)+\log(x_1)\, \times 
\nonumber \\
&
\left(\log \left(\frac{b\,s-x_{12\,}+2\,}{-b\,s-x_{12\,}+2\,}\right)+\log \left(\frac{b\,s+x_{12\,}+2\,}{-b\,s+x_{12\,}+2\,}\right)\right)
+\log \left(\frac{b\,s+x_{12\,}+2\,}{-b\,s+x_{12\,}+2\,}\right) \,\times
\nonumber \\
&
\left(-\log (x_2)-2\, \log \left(\frac{4
x_{12\,}}{x_{12\,}^2\,+4}\right)\right)
-2\, \log \left(\frac{-b\,s+x_{12\,}+2\,}{-b+x_{12\,}+2\,}\right)
\log \left(1-s\right)
\nonumber \\
&
+2\, \log \left(\frac{b\,s+x_{12\,}+2\,}{b+x_{12\,}+2\,}\right) \log \left(1-s\right)
-2\, \log \left(\frac{-b\,s+x_{12\,}+2\,}{b+x_{12\,}+2\,}\right) \log
\left(s+1\right)
\nonumber \\
&
+2\, \log \left(\frac{b\,s+x_{12\,}+2\,}{-b+x_{12\,}+2\,}\right)\,
\log \left(s+1\right)-2\,
\text{Li}_2\,\left(\frac{b-b\,s}{b-x_{12\,}+2\,}\right)
\nonumber \\
&
+2\, \text{Li}_2\,\left(\frac{b+b\,s}{b-x_{12\,}+2\,}\right)
-2\, \text{Li}_2\,\left(\frac{1}{2\,}
(-b\,s-x_{12\,})\right)
+2\, \text{Li}_2\,\left(\frac{b\,s-x_{12\,}}{2\,}\right)
\nonumber \\
&
+2\, \text{Li}_2\,\left(\frac{-b-b\,s}{-b+x_{12\,}+2\,}\right)
-2\, \text{Li}_2\,\left(\frac{b\,s-b}{-b+x_{12\,}+2\,}\right)
+2\, \text{Li}_2\,\left(\frac{b-b\,s}{b+x_{12\,}+2\,}\right)
\nonumber \\
&
-2\, \text{Li}_2\,\left(\frac{b+b\,s}{b+x_{12\,}+2\,}\right)
+2\, \text{Li}_2\,\left(\frac{-b\,s+x_{12\,}
-2\,}{b+x_{12\,}-2\,}\right)
-2\, \text{Li}_2\,\left(\frac{x_{12\,}-b\,s}{x_{12\,}-b}\right)
\nonumber \\
&
-2\, \text{Li}_2\,\left(\frac{x_{12\,}-b\,s}{b+x_{12\,}}\right)
-2\, \text{Li}_2\,\left(\frac{b\,s+x_{12\,}-2\,}{b+x_{12\,}-2\,}\right)
+2\,\text{Li}_2\,\left(\frac{b\,s+x_{12\,}}{x_{12\,}-b}\right)
\nonumber \\
&
+2\,\text{Li}_2\,\left(\frac{b\,s+x_{12\,}}{b+x_{12\,}}\right)
+ \mathcal{O}(\,\ep)
\;\Bigr]\,.
\end{align}


==> M15.tex <==
\begin{align}
\I{6} \;\;& =I_{15} = 
(s_{12})^{-2 - 2 \ep}
\frac{2^{-4 \ep} \,(1-2 \ep) \,N_{\Gamma}\,
\,(1-x_1)^{-2 \ep} \,(1-x_2)^{-2 \ep}}{x_1 \,x_2} \,\times
\nonumber \\
&
\Bigl[
+\frac{1}{2\, \ep^2}
+\frac{1}{\ep}\;\Bigl\{\text{\,H}\,(-1,x_1)+\text{\,H}\,(-1,x_2)-\text{\,H}\,(0,x_1)-\text{\,H}\,(0,x_2)\Bigr\}
\nonumber \\
&
-2 \text{\,H}\,(1,x_1)^2+4 \log\,(2) \text{\,H}\,(1,x_1)-2 \text{\,H}\,(1,x_2)^2+3 \text{G}\,(-1,-x_2,x_1)
\nonumber \\
&
-3 \text{G}\,(1,-x_2,x_1)
+\text{\,H}\,(0,x_1)
\,(2 \text{\,H}\,(0,x_2)+2 \text{\,H}\,(1,x_1))
\nonumber \\
&
+\text{\,H}\,(0,x_2)
\,(3 \text{\,H}\,(1,x_1)+2 \text{\,H}\,(1,x_2))-2 \text{\,H}\,(-1,-1,x_1)-2 \text{\,H}\,(-1,-1,x_2)
\nonumber \\
&
-\text{\,H}\,(-1,0,x_1)+2 \text{\,H}\,(-1,0,x_2)+2 \text{\,H}\,(-1,1,x_1)+2 \text{\,H}\,(-1,1,x_2)
\nonumber \\
&
-2 \text{\,H}\,(0,-1,x_1)
-2 \text{\,H}\,(0,-1,x_2)+2 \text{\,H}\,(0,0,x_1)+2 \text{\,H}\,(0,0,x_2)
\nonumber \\
&
-2 \text{\,H}\,(0,1,x_1)-2 \text{\,H}\,(0,1,x_2)-2 \text{\,H}\,(1,-1,x_1)-2 \text{\,H}\,(1,-1,x_2)
\nonumber \\
&
-\text{\,H}\,(1,0,x_1)+2 \text{\,H}\,(1,0,x_2)+4 \text{\,H}\,(1,1,x_1)
+4 \text{\,H}\,(1,1,x_2)
\nonumber \\
&
+\text{\,H}\,(-1,x_1)
\,(-\text{\,H}\,(-1,x_2)+\text{\,H}\,(0,x_2)-2 \text{\,H}\,(1,x_1)+4 \log
\,(2))
\nonumber \\
&
+\text{\,H}\,(-1,x_2)
\,(-2 \text{\,H}\,(0,x_1)-3 \text{\,H}\,(1,x_1)-2 \text{\,H}\,(1,x_2)+4 \log
\,(2))
\nonumber \\
&
+4 \text{\,H}\,(1,x_2) \log \,(2)
+\frac{3 \pi ^2}{4}+ \mathcal{O}(\ep)\,\Bigr]
\end{align}


==> M2.tex <==
\begin{align}
\I{1} \;\;&=I_2 =
(s_{12})^{- 2 \ep}
 \frac{N_{\Gamma}\, (1-x_1)\,^{-2 \ep}
(1-x_2)\,^{-2 \ep} }{(1-3\, \ep)\, \,(x_1+x_2)\,}
\nonumber \\
&
\Bigl[
+(x_1-1)\, (x_2-1)\,
+\,\ep\;\Bigl\{2 \log (2)\, (x_1+x_2)\,+2
(x_1 x_2+1)\, \text{G}(-x_2,x_1)\,
\nonumber \\
&
-(x_1-1)\, (x_2-1)\, \text{\,H}(0,x_1)\,+(x_1+1)\,
(x_2+1)\, (-\text{\,H}(-1,x_1)\,
\nonumber \\
&
-\text{\,H}(-1,x_2)\,+\text{\,H }(0,x_2)\,)\,\Bigr\}
\nonumber \\
&
+\,\ep^2\;\Bigl\{(x_1 x_2+1)\,
(-2 \text{G}(0,-x_2,x_1)\,-2 \text{G}(-x_2,-1,x_1)\,-2 \text{G}(-x_2,0,x_1)\,
\nonumber \\
&
+4\, \text{G}(-x_2,-x_2,x_1)\,+\text{G}(-x_2,x_1)\,
(2 \text{\,H}(0,x_2)\,-2 \text{\,H}(-1,x_2)\,)\,)\,
\nonumber \\
&
+(x_1-1)\, (x_2-1)\,
(-\text{\,H}(0,-1,x_2)\,+\text{\,H}(0,0,x_1)\,+\text{\,H}(0,0,x_2)\,)\,
\nonumber \\
&
+(x_2 x_1+3\,x_1+3\, x_2+1)\,
(\text{G}(1,-x_2,x_1)\,+\text{\,H}(-1,x_2)\, \text{\,H}(1,x_1)\,
\nonumber \\
&
+\text{\,H}(1,-1,x_1)\,+\text{\,H}(1,-1,x_2)\,)\,+(x_1+1)\,
(x_2+1)\, \,\times 
\nonumber \\
&
\left(-3\, \text{G}(-1,-x_2,x_1)\,-\text{\,H}(0,x_1)\, \text{\,H}(0,x_2)\,+2 \text{\,H}(-1,-1,x_1)\,+2 \text{\,H}(-1,-1,x_2)\,
\right. \nonumber \\
& \left.
+\text{\,H}(-1,0,x_1)\,-2 \text{\,H}(-1,0,x_2)\,+\text{\,H}(0,-1,x_1)\,
+\text{\,H}(-1,x_2)\,(2 \text{\,H}(-1,x_1)\,
\right.\nonumber \\
& \left.
+\text{\,H}(0,x_1)\,-\log (2)\,)\,+\text{\,H}(-1,x_1)\,
(-2 \text{\,H}(0,x_2)\,-\log (2)\,)\,-\frac{\pi ^2}{3\,}\right)\,
\nonumber \\
&
+(-x_2 x_1-3\, x_1-3\,x_2-1)\, (\text{\,H}(0,x_2)\, \text{\,H}(1,x_1)\,+\log
(2)\, \text{\,H}(1,x_1)\,
\nonumber \\
&
+\text{\,H}(1,0,x_2)\,
%\nonumber \\
%&
+\text{\,H}(1,x_2)\, \log(2)\,)\,+(x_1+x_2)\, \left(-2 \log
(2)\, \text{\,H}(0,x_1)\,
\right.\nonumber \\
& \left.
-2 \log^2(2)\,
-2 \text{\,H}(0,x_2)\, \log (2)\,\right)\,\Bigr\} + \mathcal{O}(\ep^3)\;\Bigr]
\,.
\end{align}


==> M3.tex <==
\begin{align}
% MR 10.1.2011: k_a -> k_j, k_b -> k_k
\I{6} &\times (-(k_j \cdot p_1)(k_j \cdot p_3))  \;\; =I_3
= 
(s_{12})^{1 - 2 \ep}
\frac{(1-2 \ep) \,N_{\Gamma}\, (1-x_1)^{-2 \ep}
(1-x_2)^{-2 \ep} }{8 (x_1+x_2)^2} \,\times
\nonumber \\
&
\Bigl[(x_1-1) (5 x_1-1) \text{H}(0,x_2) x_2^2-2 x_1 (x_1-x_2) \text{H}(0,x_1)
 \text{H}(0,x_2) x_2^2
\nonumber \\
&
-(x_1-1) (5 x_1-x_2) (x_2-1) x_2+x_1 (x_2-1) 
\left(-4
 x_2^2+x_1 x_2+2 x_2+x_1\right) \text{H}(0,x_1)
\nonumber \\
&
+\ep \,\Bigl\{-\left(-x_1^2+4 x_2
 x_1-6 x_1+1\right) \text{H}(0,x_1) \text{H}(0,x_2) x_2^2
+(x_1+1) (5 x_1+1)\,\times
\nonumber \\
&
 (-\text{H}(-1,x_1) \text{H}(0,x_2)-\text{H}(-1,0,x_1)
-\text{H}(0,-1,x_2)) x_2^2
+(x_1-1) (5 x_1-1)\,\times
\nonumber \\
&
 (2 \text{H}(0,1,x_2)-2 \text{H}(0,x_2) \text{H}(1,x_2)) x_2^2+x_1
 (12 \text{H}(0,x_2) \log (2)-12 \text{H}(0,x_1) \log (2)) x_2^2
\nonumber \\
&
+x_1
 (x_1-x_2) \left(-2 \text{G}(0,-x_2,0,x_1)-2 \text{G}(0,-x_2,x_1) 
\text{H}(0,x_2)
\right. \nonumber \\
& \left.
-4 \text{G}(-x_2,0,x_1) \text{H}(0,x_2)+\text{H}(0,x_2) \left(2 \text{H}(0,-1,x_1)+6 \text{H}(0,0,x_1)-4 \text{H}(0,1,x_1)
\right. \right.\nonumber \\
& \left. \left.
+\frac{5 \pi
 ^2}{6}\right)+\text{H}(0,x_1) \left(\text{H}(0,x_2)
 (4 \text{H}(1,x_1)+4 \text{H}(1,x_2))+2 \text{H}(0,-1,x_2)
\right.\right. \nonumber \\
& \left.\left.
-4 \text{H}(0,1,x_2)+\frac{\pi
 ^2}{2}\right)+2 \text{H}(0,-1,0,x_1)+2 \text{H}(0,-1,0,x_2)-2 \text{H}(0,0,0,x_2)
\right.\nonumber \\
& \left.
+3 \zeta(3)\right) x_2^2-(x_1-1) (23 x_1-5 x_2) (x_2-1) x_2-2 (5 x_1-x_2) (x_1
 x_2+1) \,\times
\nonumber \\
&
\text{G}(-x_2,x_1) x_2+(x_1+1) (5 x_1-x_2) (x_2+1)
 (\text{H}(-1,x_1)+\text{H}(-1,x_2)) x_2
\nonumber \\
&
+\left(4 x_2 x_1^2-6 x_1^2+x_2^2
 x_1-15 x_2 x_1-4 x_1+x_2^2+3 x_2\right) \text{H}(0,x_2) x_2
\nonumber \\
&
-2 (5 x_1-x_2)
 (x_1+x_2) \log (2) x_2
+\frac{1}{12} \pi ^2 \left(20 x_1 x_2^3-20 x_1^2 x_2^2+12 x_1 x_2^2-3 x_2^2
\right.\nonumber \\
& \left.
+10 x_1 x_2+5 x_1^2\right)+2 x_1 \left(-4 x_2^3+x_1 x_2^2-2
x_2-x_1\right) \text{G}(0,-x_2,x_1)
\nonumber \\
&
+\left(-4 x_1 x_2^3+6 x_1^2 x_2^2+12 x_1 x_2^2+x_2^2-2 x_1
x_2-x_1^2\right) \text{G}(-x_2,0,x_1)
\nonumber \\
&
-(x_2-1) \left(-6 x_2 x_1^2-2 x_1^2+9 x_2^2 x_1+2 x_2
x_1-x_2^2\right) \text{H}(0,x_1)
\nonumber \\
&
+\left(-4 x_1 x_2^3+6 x_1^2 x_2^2-12 x_1 x_2^2+x_2^2-2 x_1
x_2-x_1^2\right) \text{G}(-x_2,x_1) \text{H}(0,x_2)
\nonumber \\
&
+x_1 (x_2+1) \left(-4 x_2^2+x_1 x_2-2 x_2-x_1\right) \,\times
\nonumber \\
&
(-\text{H}(-1,x_2) \text{H}(0,x_1)-\text{H}(-1,0,x_2)
-\text{H}(0,-1,x_1))+x_1 (x_2-1) \,\times
\nonumber \\
&
\left(-4 x_2^2+x_1 x_2+2 x_2+x_1\right)
(-2 \text{H}(0,x_1) \text{H}(1,x_1)-3 \text{H}(0,0,x_1)
\nonumber \\
&
+\text{H}(0,0,x_2)+2 \text{H}(0,1,x_1))\Bigr\} + \mathcal{O}(\ep^2)\;\Bigr]\,.
\end{align}


==> M4.tex <==
\begin{align}
% MR 10.1.2011: k_a -> k_j, k_b -> k_k
\I{6}\times k_j \cdot p_1 \;\;& =I_4 =
(s_{12})^{ - 2 \ep}
 \frac{(1-2 \ep)\, \,N_{\Gamma}\,
(1-x_1)\,^{-2 \ep}(1-x_2)\,^{-2 \ep} }{4 (x_1+x_2)\,^2} \,\times
\nonumber \\
&
\Bigl[6 (x_1-1)\, (x_2-1)\, x_2-2 (x_1-1)\, (x_2+2)\, \text{\,H}(0,x_2)\,
x_2
\nonumber \\
&
+\text{\,H}(0,x_1)\, (2 x_2 \text{\,H}(0,x_2)\,-2 (x_2-1)\, (x_2
x_1-x_1+x_2)\,)\,
\nonumber \\
&
+\ep \;\Bigl\{12 x_2 \log (2)\, (x_1+x_2)\,+\frac{1}{6} \pi ^2 \left(8
x_1 x_2^2-2 x_2^2+4 x_1 x_2-11 x_2+5 x_1\right)\,
\nonumber \\
&
+2\,x_2 \text{\,G}(0,-x_2,0,x_1)\,+\text{\,H}(-1,x_2)\, (2 (x_2+1)\, (x_2
x_1+x_1-x_2)\, \text{\,H}(0,x_1)\,
\nonumber \\
&
-6 (x_1+1)\, x_2(x_2+1)\,)\,+\text{\,G}(0,-x_2,x_1)\, \left(2
x_2 \text{\,H}(0,x_2)\,
\right. \nonumber \\
&\left.
-4 \left(x_1x_2^2-x_2+x_1\right)\,\right)\,+\text{\,G}(-x_2,0,x_1)\, \left(4
x_2 \text{\,H}(0,x_2)\,
\right. \nonumber \\
& \left.
-2 \left(2 x_1 x_2^2+2 x_2^2-4 x_1 x_2-3
x_2+x_1\right)\,\right)\,
\nonumber \\
&
+\text{\,H}(-1,x_1)\, (2 (x_1+1)\, (x_2-2)\,
x_2 \text{\,H}(0,x_2)\,-6 (x_1+1)\, x_2 (x_2+1)\,)\,
\nonumber \\
&
+\text{\,G}(-x_2,x_1)\, \left(12 x_2\,(x_1 x_2+1)\,
\right. \nonumber \\
& \left.
-2 \left(2 x_1 x_2^2-2 x_2^2+4 x_1 x_2-3
x_2+x_1\right)\, \text{\,H}(0,x_2)\,\right)\,
\nonumber \\
&
+2 (x_1+1)\, (x_2-2)\,
x_2 \text{\,H}(-1,0,x_1)\,+2 (x_2+1)\, (x_2 x_1+x_1-x_2)\, \times
\nonumber \\
&
\text{\,H}(-1,0,x_2)\,+2\,(x_2+1)\, (x_2 x_1+x_1-x_2)\,
\text{\,H}(0,-1,x_1)\,
\nonumber \\
&
+2 (x_1+1)\, (x_2-2)\,
x_2 \text{\,H}(0,-1,x_2)\,+6 (x_2-1)\, (x_2 x_1-x_1+x_2)\, \times
\nonumber \\
&
\text{\,H}(0,0,x_1)\,-2
(x_2-1)\, (x_2 x_1-x_1+x_2)\, \text{\,H}(0,0,x_2)\,
\nonumber \\
&
-4 (x_2-1)\, (x_2
x_1-x_1+x_2)\, \text{\,H}(0,1,x_1)\,-4 (x_1-1)\, x_2 (x_2+2)\, \times
\nonumber \\
&
\text{\,H}(0,1,x_2)\,-2
x_2 \text{\,H}(0,-1,0,x_1)\,-2 x_2 \text{\,H}(0,-1,0,x_2)\,
\nonumber \\
&
+2\,x_2 \text{\,H}(0,0,0,x_2)\,+\text{\,H}(0,x_1)\, \left(-2 \text{\,H}(0,-1,x_2)\,
x_2+4 \text{\,H}(0,1,x_2)\, x_2
\right. \nonumber \\
& \left.
-4 (2 x_1-x_2)\, \log (2)\, x_2-\frac{\pi ^2
x_2}{2}-4 (x_2-1)\, (2 x_2 x_1-x_1-x_2)\,
\right.\nonumber \\
& \left.
+4 (x_2-1)\,
(x_2\,x_1-x_1+x_2)\, \text{\,H}(1,x_1)\,+\text{\,H}(0,x_2)\, \times
\right. \nonumber \\
& \left.
(-2 x_2 (x_2 x_1-2
x_1+x_2+2)\,-4 x_2 \text{\,H}(1,x_1)\,-4
x_2 \text{\,H}(1,x_2)\,)\,\right)\,
\nonumber \\
&
+\text{\,H}(0,x_2)\, \left(4 (x_1 x_2+2 x_2+3)\,
x_2+4 (x_1-1)\, (x_2+2)\, \text{\,H}(1,x_2)\, x_2
\right. \nonumber \\
& \left.
-2 \text{\,H}(0,-1,x_1)\,
x_2-6 \text{\,H}(0,0,x_1)\, x_2
\right. \nonumber \\
& \left.
+4 \text{\,H }(0,1,x_1)\, x_2+4 (2 x_1-x_2)\, \log (2)\, x_2-\frac{5 \pi ^2
x_2}{6}\right)\,
\nonumber \\
&
+x_2 (26 x_2 x_1-26 x_1-26 x_2-3 \zeta (3)\,+26)\,\Bigr\} + \mathcal{O}(\ep^2)\,\Bigr]\,.
\end{align}


==> M5.tex <==
\begin{align}
% MR 10.1.2011: k_a -> k_j, k_b -> k_k
\I{6}\times (- k_j \cdot p_3) \;\;& =I_5 = 
(s_{12})^{ - 2 \ep}
\frac{(1-2 \,\ep)\,\, N_{\Gamma} \,(1-x_1)^{-2 \,\ep}
(1-x_2)^{-2 \,\ep}}{2 \,(x_1+x_2)} \,\times
\nonumber \\
&
\Bigl[x_1 (x_2-1)\,\, \text{\,H}(0,x_1)\,\,-(x_1-1)\,\,
x_2 \text{\,H}(0,x_2)\,
\nonumber \\
&
+\,\ep \, \Bigl\{\frac{1}{12} \pi ^2 (2 x_2 x_1+5 x_1-3 x_2)\,\,
-2x_1 \text{\,G}(0,-x_2,x_1)\,\,
\nonumber \\
&
+(2 x_2 x_1-x_1+x_2)\,\, \text{\,G}(-x_2,0,x_1)\,\,
+(-2 x_2x_1-x_1+x_2)\,\times
\nonumber \\
&
\text{\,G}(-x_2,x_1)\,\, \text{\,H}(0,x_2)\,\,-(x_1+1)\,\,
x_2 \text{\,H}(-1,0,x_1)\,\,
\nonumber \\
&
+x_1 (x_2+1)\,\, \text{\,H}(-1,0,x_2)\,\,
+ x_1 (x_2+1)\,\,\text{\,H}(0,-1,x_1)\,\,
\nonumber \\
&
-(x_1+1)\,\, x_2 \text{\,H}(0,-1,x_2)\,\,
-3 x_1(x_2-1)\,\, \text{\,H}(0,0,x_1)\,\,
\nonumber \\
&
+x_1(x_2-1)\,\, \text{\,H}(0,0,x_2)\,
+2 x_1(x_2-1)\,\, \text{\,H}(0,1,x_1)\,\,
\nonumber \\
&
-2 (x_1-1)\,\,x_2 \text{\,H}(0,1,x_2)\,\,
%\nonumber \\
%&
+\text{\,H}(0,x_1)\,\, (2 x_1\,(x_2-1)\,
\nonumber \\
&
-2 x_1 \text{\,H}(1,x_1)\,\, (x_2-1)\,\,
+x_1 (x_2+1)\,\, \text{\,H}(-1,x_2)\,\,
\nonumber \\
&
+(x_1-1)\,\,x_2 \text{\,H}(0,x_2)\,\,-2 x_1 x_2 \log (2)\,\,)\,\,
\nonumber \\
&
+\text{\,H}(0,x_2)\,\, (-2 (x_1-1)\,\,
x_2-(x_1+1)\,\, \text{\,H}(-1,x_1)\,\, x_2
\nonumber \\
&
+2 (x_1-1)\,\, \text{\,H}(1,x_2)\,\, x_2
+2 x_1 x_2\,\log (2))\, \Bigr\} + \mathcal{O}(\ep^2)\;\Bigr]\,.
\end{align}


==> M6.tex <==
\begin{align}
\I{6} \;\;& =I_6 = 
(s_{12})^{-1 - 2 \ep}
\frac{(1-2 \,\ep) \,N_{\Gamma}\, (1-x_1)^{-2 \,\ep}
(1-x_2)^{-2 \,\ep}}{x_1+x_2} \,\times
\nonumber \\
&
\Bigl[\text{\,H}(0,x_1) \text{\,H}(0,x_2)
+\,\ep \,\Bigl\{\text{\,G}(0,-x_2,0,x_1)
+\text{\,G}(0,-x_2,x_1) \text{\,H}(0,x_2)
\nonumber \\
&
+2 \text{\,G}(-x_2,0,x_1) \text{\,H}(0,x_2)
+\text{\,H}(0,x_2) \left(-\text{\,H}(0,-1,x_1)
-3 \text{\,H}(0,0,x_1)
\right. \nonumber \\
& \left. 
+2 \text{\,H}(0,1,x_1)-\frac{5 \pi^2}{12}\right)
+\text{\,H}(0,x_1) \left(\text{\,H}(0,x_2)
(-2 \text{\,H}(1,x_1)-2 \text{\,H}(1,x_2))
\right. \nonumber \\
& \left.
-\text{\,H}(0,-1,x_2)
+2 \text{\,H}(0,1,x_2)-\frac{\pi^2}{4}\right)-\text{\,H}(0,-1,0,x_1)
-\text{\,H}(0,-1,0,x_2)
\nonumber \\
&
+\text{\,H }(0,0,0,x_2)
-\frac{3 \zeta (3)}{2}\Bigr\} + \mathcal{O}(\ep^2)\, \Bigr]\,.
\end{align}


==> M7.tex <==
\begin{align}
\I{7} \;\;& =I_7 = 
(s_{12})^{-1 - 2 \ep}
\frac{(1-2 \,\ep)\, N_{\Gamma} (1-x_1)\,^{-2 \,\ep}
(1-x_2)\,^{-2 \,\ep}}{x_2} \,\times 
\nonumber \\
&
\Bigl[\text{\,G}(-x_2,x_1)\,-\text{\,H}(-1,x_1)\,+\text{\,H}(0,x_2)\, 
+\ep\,\Bigl\{-3 \text{\,G}(-1,-x_2,x_1)\,
\nonumber \\
&
-\text{\,G}(0,-x_2,x_1)\,
-\text{\,G}(1,-x_2,x_1)\,-\text{\,G}(-x_2,-1,x_1)\,
-\text{\,G}(-x_2,0,x_1)\,
\nonumber \\
&
+2 \text{\,G}(-x_2,-x_2,x_1)\,
+\text{\,G}(-x_2,x_1)\,
(-\text{\,H}(-1,x_2)\,+\text{\,H}(0,x_2)\,+2)\,
\nonumber \\
&
-\text{\,H}(-1,x_2)\, \text{\,H}(1,x_1)\,
+\text{\,H}(0,x_2)\,
(-\text{\,H}(0,x_1)\,+\text{\,H}(1,x_1)\,-2 \text{\,H}(1,x_2)\,+2)\,
\nonumber \\
&
+2 \text{\,H}(-1,-1,x_1)\,
+\text{\,H}(-1,0,x_1)\,-2 \text{\,H}(-1,1,x_1)\,
\nonumber \\
&
+\text{\,H}(0,-1,x_1)\,-\text{\,H}(0,-1,x_2)\,+2 \text{\,H}(0,1,x_2)\,
-3 \text{\,H}(1,-1,x_1)\,
\nonumber \\
&
+\text{\,H}(-1,x_1)\,
(-2 \text{\,H}(0,x_2)\,+2 \text{\,H}(1,x_1)\,+\log (2)\,-2)\,
\nonumber \\
&
+\text{\,H }(1,x_1)\, \log(2)\,-\frac{\pi ^2}{4}
\Bigr\} + \mathcal{O}(\ep^2) \,\Bigr]\,.
\end{align}


==> M8.tex <==
\begin{align}
\I{8} \;\;& =I_8 = 
(s_{12})^{-1 - 2 \ep}
\frac{(1-2 \,\ep)\, N_{\Gamma}\, (1-x_1)\,^{-2 \,\ep}
(1-x_2)\,^{-2 \,\ep}}{x_1} \,\times
\nonumber \\
&
\Bigl[
+\frac{1}{\ep}\Bigl\{\text{G}(-x_2,x_1)\,-\text{\,H}(-1,x_1)\,\Bigr\}
\nonumber\\
&
-3 \text{G}(-1,-x_2,x_1)\,+2 \text{G}(0,-x_2,x_1)\,-\text{G}(1,-x_2,x_1)\,
-\text{G}(-x_2,-1,x_1)\,
\nonumber \\
&
-\text{G}(-x_2,0,x_1)\,+2 \text{G}(-x_2,-x_2,x_1)\,
\nonumber \\
&
+\text{G}(-x_2,x_1)\,
(\text{\,H}(0,x_2)\,-\text{\,H}(-1,x_2)\,)\,-\text{\,H}(-1,x_2)\,
\text{\,H}(1,x_1)\,
\nonumber \\
&
+\text{\,H}(0,x_2)\, \text{\,H}(1,x_1)\,
+2 \text{\,H}(-1,-1,x_1)\,+\text{\,H}(-1,0,x_1)\,-2 \text{\,H}(-1,1,x_1)\,
\nonumber \\
&
-2 \text{\,H}(0,-1,x_1)\,
-3 \text{\,H}(1,-1,x_1)\,+\text{\,H}(-1,x_1)\, (2 \text{\,H}(1,x_1)\,+\log
(2)\,)\,
\nonumber \\
&
+\text{\,H}(1,x_1)\, \log (2)\,+ \mathcal{O}(\ep)\,\Bigr]\,.
\end{align}


==> M9.tex <==
\begin{align}
\I{9} \;\;& =I_9 = 
(s_{12})^{-1 - 2 \ep}
\frac{(1-2 \,\ep)\, N_{\Gamma}\, (1-x_1)\,^{-2 \,\ep} 
(1-x_2)\,^{-2 \,\ep}}{x_2} \,\times
\nonumber \\
&
\Bigl[
+ \frac{1}{\,\ep}\Bigl\{\text{\,G}(-x_2,x_1)\,-\text{\,H}(-1,x_2)\,-\text{\,H}(0,x_1)\,+\text{\,H}(0,x_2)\,\Bigr\}
\nonumber \\
&
-4 \text{\,G}(0,-x_2,x_1)\,+2 \text{\,G}(1,-x_2,x_1)\,
-\text{\,G}(-x_2,-1,x_1)\,-\text{\,G}(-x_2,0,x_1)\,
\nonumber \\
&
+2 \text{\,G}(-x_2,-x_2,x_1)\,+\text{\,G}(-x_2,x_1)\,
(\text{\,H}(0,x_2)\,-\text{\,H}(-1,x_2)\,)\,
\nonumber \\
&
+\text{\,H}(0,x_1)\,(2 \text{\,H}(1,x_1)\,
-3 \text{\,H}(0,x_2)\,)\,
+\text{\,H}(0,x_2)\,
(-2 \text{\,H}(1,x_1)\,-2 \text{\,H}(1,x_2)\,)\,
\nonumber \\
&
+2 \text{\,H}(-1,-1,x_2)\,
-2 \text{\,H}(-1,0,x_2)\,-2 \text{\,H}(-1,1,x_2)\,+\text{\,H}(0,-1,x_1)\,
\nonumber \\
&
-3 \text{\,H}(0,-1,x_2)\,+3 \text{\,H}(0,0,x_1)\,
+3 \text{\,H}(0,0,x_2)\,-2 \text{\,H}(0,1,x_1)\,+2 \text{\,H}(0,1,x_2)\,
\nonumber \\
&
-3 \text{\,H}(1,-1,x_2)\,+3 \text{\,H}(1,0,x_2)\,
+\text{\,H}(-1,x_2)\,
(3 \text{\,H}(0,x_1)\,+2 \text{\,H}(1,x_1)\,
\nonumber \\
&
+2 \text{\,H}(1,x_2)\,+\log(2)\,)\,+\text{\,H}(1,x_2)\, \log (2)\,
+\frac{\pi ^2}{2} + \mathcal{O}(\,\ep)\,\Bigr]\,.
\end{align}

